Fighting Fire with Fire: Using Antidote Data to Improve Polarization and Fairness of Recommender Systems

The increasing role of recommender systems in many aspects of society makes it essential to consider how such systems may impact social good. Various modifications to recommendation algorithms have been proposed to improve their performance for specific socially relevant measures. However, previous proposals are often not easily adapted to different measures, and they generally require the ability to modify either existing system inputs, the system's algorithm, or the system's outputs. As an alternative, in this paper we introduce the idea of improving the social desirability of recommender system outputs by adding more data to the input, an approach we view as providing `antidote' data to the system. We formalize the antidote data problem, and develop optimization-based solutions. We take as our model system the matrix factorization approach to recommendation, and we propose a set of measures to capture the polarization or fairness of recommendations. We then show how to generate antidote data for each measure, pointing out a number of computational efficiencies, and discuss the impact on overall system accuracy. Our experiments show that a modest budget for antidote data can lead to significant improvements in the polarization or fairness of recommendations.

==> Heuristics.tex <==
\section{Heuristic Algorithms}

\begin{equation}
\frac{\partial R}{\partial \tilde{x}_{ij}} = \tilde{\vecu}_i^T \Sigma_j^{-1} \matU^T g_j
\end{equation}
where $\Sigma_j = \sum_{i \in \Omega^j} \vecu_i \vecu^\intercal_i + \tilde{\matU}^\intercal \tilde{\matU} + 
\lambda \matI_{\ell}$. We approximate $\tilde{\vecu}^T_i \Sigma_j^{-1} \approx \mathbbm{1}^T_j$ and set: 

\begin{equation}
\tilde{x}_{ij} = sgn(\mathbbm{1}^T_j \matU^T g_j)
\end{equation}


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g copyright statements.

==> heuristic-original.tex <==
\subsection{Heuristic Algorithms for the Fairness Utility}\label{sec:heuristics}
Before presenting results for the fairness utilities, we describe two heuristic algorithms that significantly speed up the construction of antidote data for fairness. As we will show in the next section, we see a regular pattern in the resulting antidote data generated by algorithm \ref{alg:compute-antidote-data} for our fairness utilities regardless of the initialization. (e.g., look at the antidote data generated for improving group fairness in fig.\ref{fig:group-optimal}.) In particular, we observe that:

\begin{enumerate}[label=(\roman*)]
\item Most of the users(rows) in the antidote data converge to a single rating preference of items even if they are initialized from different random values. (visible as vertical stripes in fig. \ref{fig:group-optimal}.)
\item Most of the ratings in the resulting antidote data are equal to one of the boundary values in the feasible set, i.e., they are either 0 or 5.   
\end{enumerate}

We use the above observations to design efficient heuristic algorithms for generating antidote data to improve fairness. Notice that the running time of algorithm mainly depends on the number of times that it calls function $\Thetabold$ since each evaluation of $\Thetabold$ requires solving a matrix factorization. Thus our goal is to minimize the number of calls to function $\Thetabold$.

To achieve our heuristics we exploit several approximations to algorithm  \ref{alg:compute-antidote-data}. First of all, (i) suggests that we can  approximate the antidote data by finding a single antidote user, i.e., antidote data for budget=1, and repeat the same pattern of item preferences for the given budget. Moreover, we use (ii) to approximate the antidote ratings in the first iteration of the algorithm and by considering an infinite step size. In other words, we set each antidote rating to either $\mathbb{M}_{min}$ or $\mathbb{M}_{max}$ based on the sign of the corresponding partial derivatives in the first iteration of the algorithm. Therefore, we avoid further evaluations of $\Thetabold$ required for choosing the step size. In particular, our first heuristic algorithm for minimizing utility $R$ is:

\vspace{4pt}
\textbf{\texttt{heuristic1:}}
\begin{enumerate}[label=\arabic*.]
   \item Start from a single antidote user $\tilde{\vecx}_1^{(0)}$.
   \item  Compute $\matU,\tilde{\vecu}_1,\matV = \Thetabold(\matX;\tilde{\vecx}_1^{(0)})$.
   \item Find $\frac{\partial R(\hat{\matX})}{\partial \tilde{x}_{1j}}$ for each item $j$ using eq. (\ref{eq:gradient-final}).
   \item If $\frac{\partial R(\hat{\matX})}{\partial \tilde{x}_{1j}} >0$ set $\tilde{x}_{1j} = \mathbb{M}_{min}$ Else set $\tilde{x}_{1j} = \mathbb{M}_{max}.$
   \item Copy $\tilde{\vecx}_1$ $\alpha$ times to generate $\tilde{\matX}$ for a given budget $\alpha.$ 
\end{enumerate}

Although \textbf{\texttt{heuristic1}} reduces the number of queries to function $\Thetabold$ to 1, it is still impractical in some scenarios. For example, running the matrix factorization even one more time may be expensive when working with large data, or a party may want to generate antidote data by having access to current optimal factors but not the factorization algorithm. We suggest another heuristic for such scenarios by using more approximations. 

First, we ignore the effect of adding a single antidote user on the original factors $\matU$ and $\matV$. Furthermore, by defining $\veca_j=(\vecg_j^\intercal \matU^\intercal)^\intercal$ and $\vecb_j=\matS_j^{-1} \tilde{\vecu}_1$ and using (\ref{eq:gradient-final}) we can write $\frac{\partial R(\hat{\matX})}{\partial \tilde{x}_{1j}} = \veca_j^\intercal \vecb_j$. Notice that $\veca_j$ is a weighted sum of all the user latent vectors where the weight of $\vecu_i$ is defined by $g_{ij}$, the gradient of the utility with
respect to the estimated rating $\hat{x}_{ij}$. On the other hand, $\matS_j$ is positive by definition and for a positive $\tilde{\vecu}_1$ we get a positive $\vecb_j$. Therefore, for a large enough $\lambda$ and for utility functions that yield large enough $\veca_j$, we observe that the variability of the values in $\veca_j$ are much larger than the variability of the values in $\vecb_j$ and hence we can use the approximation $\veca_j^\intercal \vecb_j \approx c \veca_j^\intercal \mathbf{1}_\ell$ where $c$ is a constant and $\mathbf{1}_\ell$ is an $\ell$-dimensional vector of $1$'s. Therefore we define our second heuristic algorithm as:

\vspace{4pt}
\textbf{\texttt{heuristic2:}}
\begin{enumerate}[label=\arabic*.]
   \item Compute $\nabla_{\hat{\matX}} R(\hat{\matX})$ and reshape it into an $n \times d$ matrix $\matG$.
%   \item Set $\tilde{x}_{1j} = -sgn(\vecg_j^\intercal \matU^\intercal \mathbf{1}_\ell)$ using $\matG$ and the original factor $\matU.$
   \item If $\vecg_j^\intercal \matU^\intercal \mathbf{1}_\ell >0$ set $\tilde{x}_{1j} = \mathbb{M}_{min}$ Else set $\tilde{x}_{1j} = \mathbb{M}_{max}.$
   \item Copy $\tilde{\vecx}_1$ $\alpha$ times to generate $\tilde{\matX}$ for a given budget $\alpha.$ 
\end{enumerate}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/individual/ind-81-True}
        \caption{Individual fairness}
        \label{fig:individual-fairness}
    \end{subfigure}
    \quad \quad
    \begin{subfigure}[]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/genres/genres-81-True}
        \caption{Group fairness}
        \label{fig:group-fairness}
    \end{subfigure}
    \caption{Improving fairness.}\label{fig:fairness}
\end{figure*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

